GlossLM: A Massively Multilingual Corpus and Pretrained Model for Interlinear Glossed Text

Language documentation projects often involve the creation of annotated text in a format such as interlinear glossed text (IGT), which captures fine-grained morphosyntactic analyses in a morpheme-by-morpheme format. However, there are few existing resources providing large amounts of standardized, easily accessible IGT data, limiting their applicability to linguistic research, and making it difficult to use such data in NLP modeling. We compile the largest existing corpus of IGT data from a variety of sources, covering over 450k examples across 1.8k languages, to enable research on crosslingual transfer and IGT generation. We normalize much of our data to follow a standard set of labels across languages. Furthermore, we explore the task of automatically generating IGT in order to aid documentation projects. As many languages lack sufficient monolingual data, we pretrain a large multilingual model on our corpus. We demonstrate the utility of this model by finetuning it on monolingual corpora, outperforming SOTA models by up to 6.6\%. Our pretrained model and dataset are available on Hugging Face.

==> tables/acc_unseg.tex <==
\begin{table*}[!htb]
\small
\centering
\resizebox{\textwidth}{!}{
    \def\arraystretch{1.2}
    \begin{tabular}{l | c c c c | c c c c c}
    \toprule
    \multirow{3}{*}{\textbf{Model}} & \multicolumn{9}{c}{Morpheme accuracy / Word accuracy (Unsegmented)} \\
    & \multicolumn{4}{c|}{\textit{In-domain}} & \multicolumn{5}{c}{\textit{Out-of-domain}} \\
    & \textbf{arp} &  \textbf{ddo} & \textbf{usp} & \textit{Avg} & \textbf{git} & \textbf{lez} & \textbf{ntu} & \textbf{nyb} & \textit{Avg} \\
    \midrule
    \textsc{Top-choice} & 27.9 / 56.9 & 15.2 / 64.1 & 43.6 / 60.4 & 28.9 / 60.5 & 3.6 / 16.9 & 20.1 / 58.2 & 12.7 / 55.1 & 72.3 / 76.7 & 27.2 / 51.7  \\
    \textsc{Token-class} & 43.6 / 69.9 & 51.2 / 74.3 & 57.2 / 72.1 & 50.7 / 72.1 &  8.54 / 16.9 & 40.7 / 45.5 & 19.4 / 48.2 & 14.2 / 5.96 & 20.7 / 29.1  \\
    \textsc{T{\"u}-CL} & 77.8 / 77.5 & 74.1 / 80.4 & 70.0 / 73.4 & 74.0 / 77.1 &  \textbf{11.7} / 21.1 & \textbf{59.9} / \textbf{71.8} & 56.2 / 78.0 & 85.2 / 85.0 & 53.3 / 64.0 \\
    \textsc{ByT5\textsubscript{unseg}} & 80.8 / 79.7 & \textbf{84.2} / \textbf{87.4} & \textbf{78.9} / \textbf{82.5} & 81.3 / 83.2 & 0.1 / 0.3 & 42.2 / 53.4 & 53.7 / 71.0 & \textbf{90.4} / \textbf{88.4} & 46.6 / 53.3  \\
    \midrule
    \textsc{GlossLM\textsubscript{unseg, pre}} & 79.8 / 79.2 & 77.5 / 82.8 & 76.8 / 80.8 & 78.0 / 80.9 & 2.3 / 3.5 & 1.5 / 1.3 & 4.1 / 9.6 & 1.6 / 2.9 & 2.4 / 4.3 \\
    \textsc{GlossLM\textsubscript{unseg, ft}} & \textbf{82.1} / \textbf{81.5} & 83.6 / 87.3 & 78.6 / 81.0 & \textbf{81.4} / \textbf{83.3} &  10.1 / \textbf{28.4}  & 57.3 / 64.9 & \textbf{62.8} / \textbf{78.9} & 87.4 / 86.2 & \textbf{56.3} / \textbf{65.0} \\
    \bottomrule
    \end{tabular}%
}
\caption{Morpheme- and word-level accuracy of on unsegmented data. Best performance per language in each setting the table is \textbf{bolded}. \textsc{GlossLM\textsubscript{unseg, pre}} refers to performance using the pretrained \textsc{GlossLM} directly, while \textsc{GlossLM\textsubscript{unseg, ft}} refers to performance after fine-tuning the pretrained model on the specific language. The \textsc{SigMoreFun} and \textsc{IMTVault-CRF} systems did not evaluate on unsegmented data.} 
\label{tab:acc_unseg}
\end{table*}

==> tables/grambank.tex <==
\begin{table*}[!htbp]
\centering
\small
\label{tab:expected_values}
\begin{tabular}{|c|p{5.5cm}|c|}
\hline
\textbf{ID} & \textbf{Feature} & \textbf{Expected - Training Avg.} \\ \hline
GB024b & Does the numeral always follow the noun in the NP? & 0.468 \\ \hline
GB193b & Are most adnominal property words placed after nouns? & 0.536 \\ \hline
GB025b & In the pragmatically unmarked order, does the adnominal demonstrative follow the noun? & 0.425 \\ \hline
GB118 & Are there serial verb constructions? & 0.4063 \\ \hline
GB130a & Is the order in intransitive clauses with a full nominal subject consistently SV? & 0.382 \\ \hline
\end{tabular}
\caption{Most underrepresented Grambank features in training data}
\label{tab:grambank}

\end{table*}

